See Further for Parameter Efficient Fine-tuning by Standing on the Shoulders of Decomposition

The rapid expansion of large foundation models within the pre-training and fine-tuning framework has underscored that larger models often yield better results. However, the scaling up of large foundation models has led to soaring costs in fine-tuning and parameter storage, rendering extensive adaptations impractical. This challenge has sparked the development of parameter-efficient fine-tuning (PEFT), which focuses on optimizing a select subset of parameters while keeping the rest fixed, significantly lowering computational and storage overheads. While recent years have witnessed a significant success in PEFT, a deep understanding of the fundamental principles behind these methods remains unexplored. To this end, here we take the first step to unify all approaches by dissecting them from a decomposition perspective. We initiate a comprehensive mathematical analysis of these methods, allowing us to delve deeply into their underlying mechanisms, and we explore the reasons behind the variations in performance among different techniques. Furthermore, inspired by our theoretical analysis, we introduce two novel PEFT methods alongside a simple yet effective framework designed to enhance the performance of PEFT techniques across various applications. Our empirical validations, conducted across multiple datasets, demonstrate the efficacy of these methods, showcasing both theoretical validity and practical performance improvements under the guidance of our analytical findings. We believe our work will deepen researchers' understanding of PEFT and other techniques, prompting further contemplation and advancing the research across the whole community.

==> sec/5.method.tex <==
\section{Methods}
\subsection{Mathematical Framework}


As discussed earlier in Section \ref{sec result overview}, PEFT methods can be viewed as different mechanisms of subspace tuning. 
We provide mathematical analyses of each method, focusing on their subspace transformations and theoretical underpinnings.

\subsection{Reconstruction-based Methods}\label{sec: reco method}

Reconstruction-based PEFT strategies focus on modifying the subspaces associated with the original weight matrix $\mathbf{W}$. 
These methods attempt to reconstruct the weight space by manipulating specific components such as singular values or singular vectors. Notable examples include SAM-PARSER \cite{peng2024sam}, Diff Pruning \cite{guo2020parameter}, (IA)$^3$ \cite{liu2022few}, BitFit \cite{zaken2021bitfit}, Prefix-tuning \cite{li2021prefix}, and Prompt-tuning \cite{lester2021power}.


Mode 1 methods adjust the singular values $\mathbf{\Sigma}'$ directly:
\begin{equation}
    \hat{\mathbf{W}} = \mathbf{U} \mathbf{\Sigma}' \mathbf{V}^{\mathsf{T}}.
\end{equation}
A representative example is SAM-PARSER \cite{peng2024sam}, which focuses on adjusting singular values in a specific portion of the network’s weight space. 
Specifically, SAM-PARSER targets the weight matrix of the SAM architecture’s ``neck'' component, which consists of two layers of dimension $256 \times 256$. 
The reconstruction process is based on optimizing the 512 singular values corresponding to these two layers. Mathematically, for a weight matrix $\mathbf{W}$, SAM-PARSER adjusts its singular values while keeping the singular vectors fixed.


Mode 2 methods adjust the singular vectors by linear or nonlinear transformations, allowing for modifications to the subspaces spanned by $\mathbf{U}$ and $\mathbf{V}$. We start from scaling the subspaces.
Let $\mathbf{D}_1 \in \mathbb{R}^{n \times n}$ and $\mathbf{D}_2 \in \mathbb{R}^{m \times m}$ be diagonal scaling matrices.

\noindent
\textbf{Scale the Column Space: }
If we scale the column space of singular vectors by assigning distinct weights to each vector, the reconstructed weight matrix $\hat{\mathbf{W}}$ can then be obtained as:
\begin{equation}
\begin{aligned}
    \hat{\mathbf{W}} &= \mathbf{U}\mathbf{D}_1\mathbf{\Sigma}  \mathbf{D}_2\mathbf{V}^\mathsf{T} \\
    & = \mathbf{U}\hat{\mathbf{\Sigma}}\mathbf{V}^\mathsf{T},
\end{aligned}
\end{equation}
where $\hat{\mathbf{\Sigma}}=\mathbf{D}_1\mathbf{\Sigma}  \mathbf{D}_2$.
Therefore, scaling the column space of singular vectors is essentially an adjustment of the singular values.

\noindent
\textbf{Scale the Row Space:}
We can also apply distinct weights to each row of the singular vectors. Consequently, the reconstructed weight matrix $\hat{\mathbf{W}}$ is articulated as follows:
\begin{equation}
\begin{aligned}
    \hat{\mathbf{W}} 
    & = \mathbf{D}_1\mathbf{U}\mathbf{\Sigma}  \mathbf{V}^\mathsf{T}\mathbf{D}_2 \\
    & =  \mathbf{D}_1\mathbf{W}\mathbf{D}_2.
\end{aligned}
\label{eq adjust the row}
\end{equation}
Thus, scaling the row space spanned by the left and right singular vectors essentially corresponds to scaling both the row and column spaces of the original weight matrix.

From this perspective, some methods can yield more in-depth explanations, such as (IA)$^3$ \cite{liu2022few}. 
In the original paper \cite{liu2022few}, this method seeks to directly modify the activations within the model by introducing a learnable vector $\mathbf{l}\in\mathbb{R}^m$ to rescale the original weight matrix. 
The transformation is implemented via the Hadamard product $\odot$, represented as $\mathbf{l}\odot\mathbf{W}$. 
However, it can equivalently be expressed as $\mathbf{W}\mathbf{D}_2$, where $\mathbf{D}_2\in\mathbb{R}^{m\times m}$ is a diagonal matrix. 
Consequently, this approach actually scales the subspace of the right singular vectors, thereby reconstructing the original weight matrix $\mathbf{W}$.

The following Mode 2 methods adopt more complex transformations: 

\noindent
\textbf{BitFit and its Derivatives:}
BitFit \cite{zaken2021bitfit} is designed to optimize solely the bias terms within a model while keeping all other parameters frozen, achieving performance comparable to full fine-tuning. Extending this concept, S-BitFit \cite{lawton2023neural} integrates Network Architecture Search (NAS) with the BitFit strategy, maintaining the structural integrity of BitFit by imposing constraints on the NAS algorithm to determine whether the gradient of the bias term should be zero.

We consider the scenario of fine-tuning the bias term of a layer. For an input $\mathbf{x}\in\mathbb{R}^{l\times n}$ with frozen weights $\mathbf{W}$ and bias term $\mathbf{b}\in\mathbb{R}^{m}$, the output of the layer is computed as follows:
\begin{equation}
    {\rm output} = \mathbf{xW} + \mathbf{1}_l\mathbf{b}^\mathsf{T},
\end{equation}
where $\mathbf{1}_l\in\mathbb{R}^{l}$ is an all-one vector.
To facilitate the integration of the bias term into the weight matrix, we can augment $\mathbf{W}$ by appending $\mathbf{b}^{\mathsf{T}}$ as an additional row. This alteration leads to the following representation:
\begin{equation}
    {\rm output} = \begin{bmatrix}
        \mathbf{x} & \mathbf{1}
    \end{bmatrix} \begin{bmatrix}
        \mathbf{W}\\
        \mathbf{b}^\mathsf{T}
    \end{bmatrix} = \hat{\mathbf{x}}\hat{\mathbf{W}},
\end{equation}
where $\mathbf{1}\in\mathbb{R}^{l}$
and $\hat{\mathbf{W}}\in\mathbb{R}^{(n+1)\times m}$ is the augmented matrix. Therefore, BitFit fundamentally involves fine-tuning each element of the final row of $\hat{\mathbf{W}}$, corresponding directly to reconstructing the row space of the augmented weight matrix.


\noindent
\textbf{Soft Prompt Derivatives:}
Soft prompt derivatives, such as Prefix-tuning \cite{li2021prefix}, and prompt-tuning \cite{lester2021power}, are prevailing in natural language processing \cite{gao2020making, tan2021msp}. Prefix-tuning introduces trainable continuous tokens, or prefixes, appended to either the input or output of a layer. These prefixes, sourced from a specific parameter matrix, remain trainable while other parameters of the pre-trained model are fixed during training. Conversely, Prompt-tuning simplifies this approach by incorporating soft prompts solely at the input layer. These prompts also originate from an independent parameter matrix and are updated exclusively through gradient descent. Both methods preserve the original model parameters, providing benefits in low-data scenarios and demonstrating potential for generalization across various tasks.

Focusing on the design rather than specific layers to place prefixes, we consider a general case where for an input $\mathbf{x}\in\mathbb{R}^{l\times n}$ and the output $\mathbf{xW}$. $l$ learnable vectors $\mathbf{P}\in\mathbb{R}^{l\times m}$, known as soft prompts, are concatenated in the following formulation:
\begin{equation}
    {\rm concat}(\mathbf{P}, \mathbf{xW}) = \begin{bmatrix}
        \mathbf{P} \\ \mathbf{xW}
    \end{bmatrix}.
    \label{eq soft prompt}
\end{equation}

Similar to the approach used for BitFit, we can augment the weight matrix to restate equation (\ref{eq soft prompt}) as 
\begin{equation}
   \begin{bmatrix}
        \mathbf{P} \\ \mathbf{xW}
    \end{bmatrix} =  \begin{bmatrix}
        \mathbf{I} & \mathbf{0}_{l\times n} \\
        \mathbf{0}_{l\times l} & \mathbf{x}
    \end{bmatrix}
    \begin{bmatrix}
        \mathbf{P} \\ \mathbf{W} 
    \end{bmatrix}= \hat{\mathbf{x}}\hat{\mathbf{W}}.
\end{equation}
Here, $\mathbf{I}\in\mathbb{R}^{l\times l}$ is the identity matrix, $\mathbf{0}_{l\times n}\in\mathbb{R}^{l\times n}$ and $\mathbf{0}_{l\times l}\in\mathbb{R}^{l\times }$ are zero matrices, and $\hat{\mathbf{W}}\in\mathbb{R}^{(n+l)\times m}$ is the augmented matrix. 
Thus, soft prompt derivatives essentially involve adjusting the elements of the initial several rows of the augmented weight matrix $\hat{\mathbf{W}}$, thereby reconstructing the original subspace.

\noindent
\textbf{Others:}
There are also methods that adjust the singular vectors by directly modifying elements within the original weight matrix, such as Diff pruning \cite{guo2020parameter}, FishMask \cite{sung2021training}, Fish-Dip \cite{das2023unified}, Xattn Tuning \cite{gheini2021cross}, SPT \cite{he2023sensitivity}, and PaFi \cite{liao2023parameter}, etc.





\subsection{Extension-based Methods}
There are two prominent series of extension-based methods within parameter-efficient tuning. The first series, known as LoRA derivatives, includes developments such as LoRA \cite{hu2021lora}, AdaLoRA \cite{zhang2022adaptive}, TriLoRA \cite{feng2024trilora}, FLoRA \cite{si2024flora}, VeRA \cite{kopiczko2023vera}, and LoTR \cite{bershatsky2024lotr}. These methods primarily rely on low-rank matrix decomposition techniques. The second series, the Adapter derivatives, comprises methods such as those introduced by Houlsby et al. \cite{houlsby2019parameter}, He et al. \cite{he2021towards}, and AdapterFusion \cite{pfeiffer2020adapterfusion}, which incorporate small-scale neural modules, or adapters, into existing architectures. In the following sections, we will delve into the underlying mathematical principles of these methods and attempt to elucidate why they exhibit varying degrees of effectiveness across different applications.





\subsubsection{LoRA Derivatives and Insights Beyond}\label{sec method lora}

As shown in Section \ref{sec result lora}, methodologies such as LoRA, AdaLoRA, TriLoRA, and FLoRA incorporate the addition term $\Delta\mathbf{W}$ using various decomposition forms. 
We first demonstrate that different decomposition forms are capable of being transformed into one another. 
Using the general form of $\Delta\mathbf{W} = \mathbf{AGB}$, we have
\begin{equation}
\begin{aligned}
    & \mathbf{AMB} = \mathbf{{AU}\Sigma {VB}} \ (\mathbf{M} = \mathbf{U\Sigma V}) \\
    = & {\mathbf{A}^{\diamond}\mathbf{D}}\mathbf{B}^{\diamond} \ (\mathbf{A}^{\diamond}=\mathbf{AU}, \mathbf{B}^{\diamond}=\mathbf{VB}) \\ =&  \mathbf{A}^{*}\mathbf{B}^{\diamond} \ \ \ \ (\mathbf{A}^{*}=\mathbf{A}^{\diamond}\mathbf{D}).
\end{aligned}
\label{eq same decomposition formulation}
\end{equation}
Based on Proposition \ref{proposition 1}, even though it is possible to transform one decomposition form into another, significant differences in effectiveness will still persist.
To further elaborate on this point, let $\Delta\mathbf{W}^{*} = \mathbf{W}^{*} - \mathbf{W}$ and ideally $\mathbf{A}\mathbf{G}\mathbf{B} = \Delta\mathbf{W}^{*}$, we have $\mathbf{G} = \mathbf{A}^{\dagger}\Delta\mathbf{W}^{*}\mathbf{B}^{\dagger}$.
We utilize SVD on $\Delta\mathbf{W}^{*}$, resulting in the following expression: 
\begin{equation}
\mathbf{G} = \mathbf{A}^{\dagger} \mathbf{U} \mathbf{\Sigma} \mathbf{V}^T \mathbf{B}^{\dagger}.
\end{equation}
Suppose $\mathbf{A}^{\dagger}$ and $\mathbf{B}^{\dagger}$ as
\begin{equation}
    \mathbf{A}^{\dagger} = \mathbf{P}\mathbf{U}^\mathsf{T}, \mathbf{B}^{\dagger} = \mathbf{V}\mathbf{\Sigma}^{\dagger}\mathbf{Q},
    \label{eq a-1 b-1 compli}
\end{equation}
where $\mathbf{P}\in\mathbb{R}^{r\times n}$ and $\mathbf{Q}\in\mathbb{R}^{n\times r}$ are arbitrary matrices. Therefore, we can derive
\begin{equation}
    \mathbf{G} = \mathbf{PQ}.
\end{equation}
If $\mathbf{G}$ is an identity matrix, $\mathbf{Q}$ must be the pseudo-inverse of $\mathbf{P}$. 
Building on this setup, if $\mathbf{G}$ is a diagonal matrix, it further specifies that each column of $\mathbf{Q}$, which is the pseudo-inverse of $\mathbf{P}$, may have distinct weights. 
Conversely, when $\mathbf{G}$ is an arbitrary matrix, it does not impose any such constraints.
Therefore, we can arrive at the conclusion: LoRA imposes the most restrictions on the matrix patterns for model learning, followed by AdaLoRA, while FLoRA imposes the least.




To further ease the training process, we can introduce regularization terms that impose constraints on the matrix patterns. These regularizations help guide the learning dynamics by controlling the flexibility of the model and preventing overfitting.
Given that $\mathbf{G}$ is a diagonal matrix, we simply constrain $\mathbf{A}^{\dagger}$ and $\mathbf{B}^{\dagger}$ as
\begin{equation}
    \mathbf{A}^{\dagger} = \mathbf{D}_1\mathbf{U}^\mathsf{T}, \mathbf{B}^{\dagger} = \mathbf{V}\mathbf{D}_2,
    \label{eq a-1 b-1 simple}
\end{equation}
where $\mathbf{D}_1\in\mathbb{R}^{r\times n}$ and $\mathbf{D}_2\in\mathbb{R}^{m\times r}$ are rectangular diagonal matrices. This setup inversely dictates the formulations for $\mathbf{A}$ and $\mathbf{B}$ based on the pseudo-inverses of $\mathbf{D}_1$ and $\mathbf{D}_2$, as shown
\begin{equation}
    \mathbf{A} = \mathbf{U}\mathbf{D}_1^{\dagger}, \mathbf{B} = \mathbf{D}_2^{\dagger}\mathbf{V}^{\mathsf{T}}.
\end{equation}
This analysis reveals that $\mathbf{A}$ and $\mathbf{B}$ must be structured as linear combinations of the columns of $\mathbf{U}$ and $\mathbf{V}$, respectively. Consequently, the matrix relationships are captured as follows:
\begin{equation}
    \begin{aligned}
        \mathbf{A}\mathbf{A}^{\mathsf{T}} = \mathbf{U}\mathbf{D}_1^{\dagger}\mathbf{D}_1^{\dagger\mathsf{T}}\mathbf{U}^{\mathsf{T}}, &  \ \mathbf{A}^{\mathsf{T}}\mathbf{A} = \mathbf{D}_1^{\dagger\mathsf{T}}\mathbf{D}_1^{\dagger},\\
        \mathbf{B}^{\mathsf{T}}\mathbf{B} = \mathbf{V}\mathbf{D}_2^{\dagger\mathsf{T}}\mathbf{D}_2^{\dagger}\mathbf{V}^{\mathsf{T}}, & \ \mathbf{B}\mathbf{B}^{\mathsf{T}} = \mathbf{D}_2^{\dagger}\mathbf{D}_2^{\dagger\mathsf{T}}.
    \end{aligned}
    \label{eq aat bbt}
\end{equation}
By simplifying the constraints on $\mathbf{D}_1 = \mathbf{I}_{r\times n}\in\mathbb{R}^{r\times n}$ and $\mathbf{D}_2 = \mathbf{I}_{m\times r}\in\mathbb{R}^{m\times r}$ during training, the following identities hold:
\begin{equation}
\mathbf{D}_1^{\dagger\mathsf{T}}\mathbf{D}_1^{\dagger}=\mathbf{D}_2^{\dagger}\mathbf{D}_2^{\dagger\mathsf{T}} = \mathbf{I}_{r}.
\end{equation}  
In this configuration, $\mathbf{D}_1^{\dagger}\mathbf{D}_1^{\dagger\mathsf{T}}$ and $\mathbf{D}_2^{\dagger\mathsf{T}}\mathbf{D}_2^{\dagger}$ function as block diagonal identity matrices. This arrangement introduces a degree of semi-orthogonality to both $\mathbf{A}$ and $\mathbf{B}$, since
$\mathbf{A}^{\mathsf{T}}\mathbf{A}=\mathbf{B}\mathbf{B}^{\mathsf{T}} =\mathbf{I}_{r}$ and $\mathbf{A}\mathbf{A}^{\mathsf{T}}$ and $\mathbf{B}^\mathsf{T}\mathbf{B}$ are arbitrary matrices. 
Therefore, when $\mathbf{G}$ is a diagonal matrix, we can impose semi-positive definite constraints on matrices $\mathbf{A}$ and $\mathbf{B}$ by introducing regularization terms, as shown in equation (\ref{eq adalora constraint orthogonal}). 

Extending this further, when $\mathbf{G}$ is an identity matrix, we obtain
\begin{equation}
    \mathbf{I} = \mathbf{A}^{\dagger}\Delta\mathbf{W}^{*}\mathbf{B}^{\dagger}  = \mathbf{D}_1\mathbf{\Sigma}\mathbf{D}_2.
    \label{eq lora method analysis final}
\end{equation}
It becomes evident that $\mathbf{D}_1$ and $\mathbf{D}_2$ are intricately correlated. Therefore, it is feasible to first impose a semi-positive definite constraint to one of $\mathbf{A}$ and $\mathbf{B}$, such as $\mathbf{A}$.
As for $\mathbf{B}$, there are two possible approaches. 
First, if we assume that $\mathbf{\Sigma}$ is an identity matrix, we can also impose a semi-positive definite constraint on $\mathbf{B}$. 
This is a strong assumption and thus such regularization is an aggressive form. 
Alternatively, we can relax the constraint. Equations (\ref{eq aat bbt}) and (\ref{eq lora method analysis final}) suggest that $\mathbf{B}^\mathsf{T}\mathbf{B}$ is a diagonal matrix, and hence, we can impose a diagonal constraint on $\mathbf{B}$, as shown in equation (\ref{eq lora constraint diagonal}).

Furthermore, we can directly break the connection between $\mathbf{D}_1$ and $\mathbf{D}_2$, that is, between $\mathbf{A}$ and $\mathbf{B}$. 
This can be achieved by introducing a nonlinear operation between the multiplication of matrices $\mathbf{A}$ and $\mathbf{B}$, as illustrated in equation (\ref{eq adapter mpc}). These constraints on the matrix patterns can significantly improve the performance of LoRA.



\subsubsection{Adapter Derivatives}\label{sec adapter}

Adapter derivatives \cite{houlsby2019parameter, pfeiffer2020adapterfusion, he2021towards}, as a pioneering approach in PEFT, integrate small neural modules to adapt models effectively. These adapters, which mainly consist of a down-projection followed by an up-projection, modify only specific parts of the model during training.
For an input $\mathbf{x}\in\mathbb{R}^{n\times m}$, the adapters are integrated with a residual connection, resulting in the final transformation:
\begin{equation}
    \mathbf{x} \rightarrow \mathbf{x} +  h(\mathbf{xA})\mathbf{B},
    \label{eq adapeter}
\end{equation}
where $h(\cdot)$ is a nonlinear activation function, $\mathbf{A}\in\mathbb{R}^{m\times r}$ and  $\mathbf{B}\in\mathbb{R}^{r\times m}$. This configuration can be further expressed by considering weight matrix as the input $\hat{\mathbf{W}} = \mathbf{x}\in\mathbb{R}^{n\times m}$ and a hypothetical input $\hat{\mathbf{x}} = \mathbf{I}\in\mathbb{R}^{m\times m}$ as 
\begin{equation}
\hat{\mathbf{W}}\hat{\mathbf{x}}\rightarrow \hat{\mathbf{W}}\hat{\mathbf{x}} +h(\hat{\mathbf{W}} \mathbf{A})\mathbf{B}\hat{\mathbf{x}},
    \label{eq adapter trans}
\end{equation}
Therefore, the addition term introduced by the Adapter can be formulated as $\Delta\mathbf{W} = h(\hat{\mathbf{W}}\mathbf{A})\mathbf{B}$. Following a similar analysis in Sec. \ref{sec method lora}, we can derive
\begin{equation}
    h(\hat{\mathbf{W}}\mathbf{A}) = \Delta\mathbf{W}^{*}\mathbf{B}^{\dagger}.
\end{equation}



Innovations such as the MAM Adapter \cite{he2021towards} including PA or Scaled PA, use a parallel architecture similar to LoRA to configure adapter layers. Specifically, for an input $\mathbf{x}\in\mathbf{R}^{d\times n}$, we have
\begin{equation}
    \mathbf{x}\mathbf{W} \rightarrow \mathbf{x}\mathbf{W} + h(\mathbf{xA})\mathbf{B},
    \label{eq adapter mpc}
\end{equation}
where $\mathbf{A}\in\mathbb{R}^{n\times r}$ and  $\mathbf{B}\in\mathbb{R}^{r\times m}$. Following equation (\ref{eq adapter trans}), we have
\begin{equation}
     \hat{\mathbf{W}}\hat{\mathbf{x}} \rightarrow \hat{\mathbf{W}}\hat{\mathbf{x}}  + h(\hat{\mathbf{W}}\mathbf{A})\mathbf{B},
\end{equation}
resulting in $\Delta\mathbf{W} = h(\hat{\mathbf{W}}\mathbf{A})\mathbf{B}\hat{\mathbf{x}}^{\dagger}$. 




\subsection{Combination-based Methods}\label{sec method combination}

DoRA \cite{liu2024dora} and Spectral Adapter \cite{zhang2024spectral} are two representative combination-based methods.

DoRA \cite{liu2024dora} first decomposes the model weights $\mathbf{W}$ into two parts: magnitude and direction. The process of adjusting these components is defined as follows:
\begin{equation}
    \phi(\mathbf{W}) = \mathbf{m} \frac{\mathbf{W} + \mathbf{AB}}{\|\mathbf{W} + \mathbf{AB}\|_c},
    \label{eq Dora}
\end{equation}
where $\mathbf{m}\in\mathbb{R}^{1\times m}$ represents the magnitude, and $\|\cdot\|_c$ is the vector-wise norm of a matrix applied across each column. Given that $\mathbf{m}$ is learnable during the training process, this formula can be simplified as:
\begin{equation}
    \phi(\mathbf{W}) = \mathbf{W}\mathbf{D} + \mathbf{ABD},
\end{equation}
where $\mathbf{D}\in\mathbb{R}^{m\times m}$ is a diagonal matrix.

We focus on the extension $\Delta\mathbf{W} = \mathbf{ABD}$ while disregarding the transformation of the column space of $\mathbf{W}$. Following the analysis similar to that for LoRA derivatives, we can derive
\begin{equation}
    \mathbf{I} = \mathbf{A}^{\dagger}\Delta\mathbf{W}^{*}\mathbf{D}^{\dagger}\mathbf{B}^{\dagger} = \mathbf{A}^{\dagger}\mathbf{U}\mathbf{\Sigma}\mathbf{V}^{\mathsf{T}}\mathbf{D}^{\dagger}\mathbf{B}^{\dagger}.
\end{equation}
With the constraints $\mathbf{A}^{\dagger} = \mathbf{D}_1\mathbf{U}^\mathsf{T}$ and $\mathbf{D}^{\dagger}\mathbf{B}^{\dagger} = \mathbf{V}\mathbf{D}_2$, where $\mathbf{D}_1\in\mathbb{R}^{r\times n}$ and $\mathbf{D}_2\in\mathbb{R}^{m\times r}$ are rectangle diagonal, we have 
\begin{equation}
     \mathbf{I} = \mathbf{D}_1\mathbf{\Sigma} \mathbf{D_2}, \ \mathbf{A} = \mathbf{U}\mathbf{D}_1^{\dagger}, \ \mathbf{B}= \mathbf{D}_2^\dagger\mathbf{V}^\mathsf{T}\mathbf{D}^\dagger.
\end{equation}
It is important to note
\begin{equation}
    \mathbf{B}^\mathsf{T}\mathbf{B} = \mathbf{D}^{\dagger\mathsf{T}}\mathbf{V}\mathbf{D}_2^{\dagger\mathsf{T}} \mathbf{D}_2^\dagger\mathbf{V}^\mathsf{T}\mathbf{D}^\dagger, \  \mathbf{B}\mathbf{B}^\mathsf{T} = \mathbf{D}_2^\dagger\mathbf{V}^\mathsf{T}\mathbf{D}^\dagger\mathbf{D}^{\dagger\mathsf{T}}\mathbf{V}\mathbf{D}_2^{\dagger\mathsf{T}}.
\end{equation}
Since ${\rm rank}(\mathbf{D}_2^\dagger) =r$ and the matrix product $\mathbf{D}_2^{\dagger\mathsf{T}} \mathbf{D}_2^\dagger \in \mathbb{R}^{m\times m} $ cannot be an identity matrix, both $\mathbf{B}^\mathsf{T}\mathbf{B}$ and $\mathbf{B}\mathbf{B}^\mathsf{T}$ are arbitrary matrices. 
Therefore, DoRA can at most impose semi-orthogonal constraints on matrix $\mathbf{A}$, while matrix $\mathbf{B}$ remains unconstrained.
Additionally, DoRA reconstructs $\mathbf{W}$ by scaling its column space.

Spectral Adapter \cite{zhang2024spectral}, a combination-based method, starts by decomposing the weight matrix $\mathbf{W}$ into its SVD components $\mathbf{W} = \mathbf{U}\mathbf{\Sigma}\mathbf{V}^\mathsf{T}$. It then integrates trainable matrices $\mathbf{A}\in\mathbb{R}^{n\times r}$ and $\mathbf{B}\in\mathbb{R}^{m\times r}$ with the top r columns of $\mathbf{U}$ and $\mathbf{V}$, with the form as
\begin{equation}
    \phi(\mathbf{W}) = \begin{bmatrix}
        \mathbf{U}_r + \mathbf{A} & \mathbf{U}_{n-r}
    \end{bmatrix} \mathbf{\Sigma}  \begin{bmatrix}
        \mathbf{V}_r + \mathbf{B} & \mathbf{V}_{n-r}
    \end{bmatrix}^{\mathsf{T}},
    \label{eq spectral vector}
\end{equation}
where $\mathbf{U}_r$ and $\mathbf{V}_r$ represent the top $r$ columns of $\mathbf{U}$ and $\mathbf{V}$, and $\mathbf{U}_{n-r}$ and $\mathbf{V}_{n-r}$ account for the remaining columns. The equation (\ref{eq spectral vector}) can be rewritten as 
\begin{equation}
    \phi(\mathbf{W}) = \mathbf{W} + \mathbf{A}\mathbf{\Sigma}\mathbf{V}^\mathsf{T} + \mathbf{U}\mathbf{\Sigma}\mathbf{B}^\mathsf{T} + \mathbf{A}\mathbf{\Sigma}\mathbf{B}.
\end{equation}
Therefore, Spectral Adapter can also be viewed as introducing an additional term $\Delta\mathbf{W} = \mathbf{A}\mathbf{\Sigma}\mathbf{V}^\mathsf{T} + \mathbf{U}\mathbf{\Sigma}\mathbf{B}^\mathsf{T} + \mathbf{A}\mathbf{\Sigma}\mathbf{B}$.


SVDiff \cite{han2023svdiff} modifies the singular values $\mathbf{\Sigma}$ of the original weight matrix $\mathbf{W}$ by incorporating a diagonal “spectral shift” matrix $\mathbf{D}$. This adjustment is formulated as follows:
\begin{equation}
\phi(\mathbf{W}) = \mathbf{U} h(\mathbf{\Sigma} + \mathbf{D})\mathbf{V}^\mathsf{T},
\label{eq svdiff}
\end{equation}
where $\mathbf{U}$ and $\mathbf{V}$ represent the left and right singular vectors of $\mathbf{W}$, respectively, and $h(\cdot)$ denotes the nonlinear function ReLU. This equation can be expanded to
\begin{equation}
\begin{aligned}
\phi(\mathbf{W}) & = \mathbf{U}\mathbf{\Sigma}\mathbf{V}^\mathsf{T} + \mathbf{U}\ \mathcal{H}_\mathbf{\Sigma}(\mathbf{D})\mathbf{V}^\mathsf{T}\\
& = \mathbf{W} + \Delta\mathbf{W}.
\end{aligned}
\end{equation}
In this context, $\mathcal{H}_\mathbf{A}(\cdot)$ is an element-wise operator where $\mathcal{H}_\mathbf{\Sigma}(\mathbf{D}) = [\max(D{ij}, -\Sigma_{ij})]_{n\times m}$. Consequently, SVDiff not only reconstructs but also extends the subspace. Moreover, we can conclude that the approach, which selectively reconstructs the singular values or vectors by introducing additional trainable components rather than directly altering the singular components, can be categorized as a combination-based method.




\subsection{Implementation Details}

In our experiments, we employed three distinct scales of models: RoBERTa-base \cite{liu2019roberta}, DeBERTaV3-base \cite{he2021debertav3}, and RoBERTa-Large \cite{liu2019roberta}. We used the General Language Understanding Evaluation (GLUE) \cite{wang2018glue} benchmark as our dataset, which comprises two single-sentence classification tasks, three similarity and paraphrase tasks, and three natural language inference tasks. 
Details of the GLUE dataset are provided in Supplementary Table \ref{tab: glue dataset}.


The configurations and hyper-parameters for all methods were adopted according to their respective original publications. Specifically, (IA)$^3$ was applied to the keys and values in both self-attention and encoder-decoder attention mechanisms, as well as to the intermediate activation of the position-wise feed-forward networks, along with SSL and SSB\footnote{Following recommendations in \cite{liu2022few}, applying (IA)$^3$ to these layers is deemed sufficient.}. 
Additionally, we set the rank $r$ values at 2, 4, 8, 16 for LoRA, TriLoRA, AdaLoRA, FLoRA, and DoRA, and align the parameter budgets of other methods as closely as possible with LoRA to ensure comparability across different approaches\footnote{Previous studies such as \cite{hu2021lora} have shown that a small rank $r$ in LoRA can achieve excellent results, often surpassing those obtained with larger ranks. Therefore, we do not take a larger rank $r$ into consideration in our experiments.}. These methods were applied to all linear layers.
We conducted all baseline comparisons using the publicly available PyTorch implementation \cite{paszke2019pytorch}, and all experiments were performed on NVIDIA A100 GPUs. Results are reported as the mean of 5 runs with different random seeds to ensure the reliability and reproducibility of our findings. The hyper-parameters for different experiments are shown in Supplementary Table \ref{tab:training detail}.

==> sec/declaration.tex <==
\newpage


\section*{Declarations}


\subsection*{Competing Interests}
The authors declare no competing interests.


\subsection*{Ethics Approval}
Not applicable.

\subsection*{Consent to Participate}
Not applicable.

\subsubsection*{Consent for publication}
Not applicable.

\subsection*{Data and Material Availability}
Datasets MNLI, SST-2, CoLA, QQP, QNLI, RTE, MRPC, and STS-B used in this study are freely available at \url{https://huggingface.co/datasets/glue}.

\section*{Code Availability}
The source code of this study is publicly available on GitHub at
\url{https://github.com/Chongjie-Si/Subspace-Tuning}.



\section*{Author Contributions}
W. S. and C. S. conceived the project. C. S. performed the theoretical analysis and all experiments. C. S. wrote the paper. C. S. and W. S. checked the formulation and revised the paper. X. Y. supervised the project.



\newpage
